Learning Robust, Transferable Sentence Representations for Text Classification

Despite deep recurrent neural networks (RNNs) demonstrate strong performance in text classification, training RNN models are often expensive and requires an extensive collection of annotated data which may not be available. To overcome the data limitation issue, existing approaches leverage either pre-trained word embedding or sentence representation to lift the burden of training RNNs from scratch. In this paper, we show that jointly learning sentence representations from multiple text classification tasks and combining them with pre-trained word-level and sentence level encoders result in robust sentence representations that are useful for transfer learning. Extensive experiments and analyses using a wide range of transfer and linguistic tasks endorse the effectiveness of our approach.

==> figure.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{figure}
\vspace{-2mm}
\centering
\subfloat
{
\hspace*{-0.5cm}
\includegraphics[width=.5\linewidth]{images/sick_e_efficiency.png}
}
\subfloat
{
\includegraphics[width=.5\linewidth]{images/sst_efficiency.png}
}
\caption{Comparing performance of sentence representations and contextualized vectors on SST and SICK-E tasks as the training dataset size is varied. Sent2vec refers to the shared encoder in the shared-private MTL models.}
\label{sample_sicke}
% \vspace{-2mm}
\end{figure}


\begin{figure}
\vspace{-2mm}
\centering
\subfloat[\label{fig:rsub1}]
{
\hspace*{-0.5cm}
\includegraphics[width=.5\linewidth]{images/cove_vs_sent2vec.png}
}
\subfloat[\label{fig:rsub2}]
{
\includegraphics[width=.5\linewidth]{images/mtl_encoders.png}
}
\caption{
(a) Weights learned by transfer tasks for contextualized vectors (ELMo, CoVe), and sentence vectors which refer to a concatenation of all the private and shared encoders of the adversarial shared-private multi-task model.
(b) Weights learned by the transfer tasks for private (task-specific) and shared encoders of adversarial shared private multi-task model. }
\label{taskvsencoder}
% \vspace{-2mm}
\end{figure}


% \begin{figure}[t]
% \centering
% \includegraphics[width=0.9\linewidth]{images/cove_vs_sent2vec.png}
% \vspace{-2mm}
% \caption{Weights learned by transfer tasks for contextualized vectors (ELMo, CoVe), and sentence vectors which refer to a concatenation of all the private and shared encoders of the adversarial shared-private multi-task model.}
% \label{taskvsencoder}
% \vspace{-2mm}
% \end{figure}


% \begin{figure}[t]
% \vspace{-2mm}
% \centering
% \includegraphics[width=0.9\linewidth]{images/mtl_encoders.png}
% \vspace{-2mm}
% \caption{Weights learned by the transfer tasks for private (task-specific) and shared encoders of adversarial shared private multi-task model.}
% \label{mtlencoders}
% \vspace{-2mm}
% \end{figure}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> table/polysemous.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%\begin{table*}[]
%\centering
%\caption{Nearest Sentences to Selected Semcor Sentences}
%\label{my-label}
%\begin{tabular}{l|l}
%\hline
% Source Sentence                                                                                                                                                                      
% & Nearest Sentence                                                                                                                              \\ \hline
%\multirow{2}{*}{(A)SP} & 
%\begin{tabular}[c]{@{}l@{}}\{...\} the movies are at heart a form of fiction,\\ like the \underline{play}, the novel, or the short story.\end{tabular} & \begin{tabular}[c]{@{}l@{}}\{...\} worthy of being explored either in the \\novel or in the \underline{play} or in comedy and satire.\end{tabular}        \\ \cline{2-3} 
%                             & \begin{tabular}[c]{@{}l@{}}\{...\} Ed Keegan did the mound chores for the club down \\ from West Palm Beach to \underline{play} the game \\before 767 paying customers\{...\}  \end{tabular}                                                     & \begin{tabular}[c]{@{}l@{}}The Texans have two more road games \\ \{...\} before they \underline{play} for the home folks again, \{...\}   \end{tabular}                          \\ \hline
%\multirow{2}{*}{MTL Encoder} & A spectator picked up the ball and handed it to a small boy, who dropped this suddenly hot potato in a very playable \underline{lie}.                                                           & \{...\} even when it is finally the only thing in the world you have left to believe , and the whole world is telling you that one was a \underline{lie}. \\ \cline{2-3} 
%                             & He no longer had to \underline{lie} in his bunk all night, his eyes closed, pretending to sleep.                                                                                                & I do it, lots of times - I like to \underline{lie} in a hammock at night, by myself, when it's all quiet.                                                 \\ \hline
%\multirow{2}{*}{MTL ncoder}  & It tends to \underline{support} the longstanding precious sentiments, the traditional ways of thinking, and the customary ways of living.                                                       & Thus, the client receives enough ego \underline{support} to engage in constructive efforts on his own behalf.                                             \\ \cline{2-3} 
%                             & Finally, a balance must be effected among project finance, utilization of agricultural surpluses, and general balance of payments \underline{support}.                                          & The local community maintains responsibility for the financial \underline{support} of its own library program, facilities, and services, \{...\}          \\ \hline
%\end{tabular}
%\end{table*}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[]
\small
\centering
\begin{tabular}{p{7.5cm}|p{7.5cm}}
\hline
\multicolumn{1}{c|}{\textbf{Source Sentence}} & \multicolumn{1}{c}{\textbf{Nearest Neighbor}} \\ \hline
% \{...\} the movies are at heart a form of fiction, like the \underline{play}, the novel, or the short story.                         & \{...\} worthy of being explored either in the novel or in the \underline{play} or in comedy and satire.                           \\ \hline
% \{...\} did the mound chores from West Palm Beach to \underline{play} the game before 767 paying customers \{...\}                   & The Texans have two more road games - at Buffalo and Houston - before they \underline{play} for the home folks again, \{...\}      \\ \hline
% \{...\} a small boy, who dropped this suddenly hot potato in a very playable \underline{lie}.                                        & \{...\} and the whole world is telling you that one was a \underline{lie}.                                                         \\ \hline
% He no longer had to \underline{lie} in his bunk all night, his eyes closed, pretending to sleep.                                     & I do it, lots of times - I like to \underline{lie} in a hammock at night, by myself, when it's all quiet.                          \\ \hline
 He may \underline{support} China (but he won't); he may break with China (which would be infernally difficult and perhaps disastrous), \{...\}                      & The Chinese, North Vietnamese and North Koreans, on the other hand, feel that, militarily, Russia is strong enough to \underline{support} them in the ``just wars of liberation'' \{...\}                  \\ \hline
\{...\} effected among project finance,  utilization of agricultural surpluses, and general balance of payments \underline{support}. & The local community maintains responsibility for the financial \underline{support} of its own library program, facilities, \{...\} \\ \hline
\end{tabular}
\caption{Nearest neighbors to ``support'' using sentence embeddings from shared-private MTL models. The source and nearest neighbor sentences are picked from the SemCor 3.0 dataset.}
\label{polysemous}
\end{table*}

==> table/table2.tex <==
\begin{table}[ht]
\centering
\small
\begin{tabular}{l|c@{\hskip 0.1in} c@{\hskip 0.1in}| c@{\hskip 0.1in} c@{\hskip 0.1in}| c@{}}
\hline
& \multicolumn{2}{c|}{PTB} & \multicolumn{2}{c|}{ROCStories} & Senseval-3 \\ 
& N & $\mbox{S}_{Avg}$  & N & $\mbox{S}_{Avg}$ & N\\
\hline
Train   & 39,832 & 25.5 & 45,496 & 10.2 & 7,860 \\ 
Dev	    & 1,700 & 25.1 & 1,871 & 10.1 & - \\
Test    & 2,416 & 25.1 & 1,871 & 10.1 & 3,944 \\
\hline
\end{tabular}
\caption{Statistics of the auxiliary task datasets. For ROCStories, N indicates the number of stories and for PTB and Senseval-3, N indicates the number of sentences. $\mbox{S}_{Avg}$ is the average sentence length. For ROCStroies, spring 2016 version is used in the experiments.
}
\label{table:aux_data_stat}
% \vspace{-2mm}
\end{table}

==> table/table3.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table}[ht]
\centering
% \resizebox{\linewidth}{!}{%
\small
\begin{tabular}{@{}l@{\hskip 0.1in} c@{\hskip 0.1in} c@{\hskip 0.1in} c@{}}
\hline
Model Type & QQP & SNLI & Multi-NLI \\
% \hline 
% \citet{conneau2017supervised} & - & 84.5 & - \\
\hline\hline 
\multicolumn{4}{l}{1. In domain single task sentence representation learning} \\ 
% \hline
1.1 BiLSTM-Max & 86.7 & 84.5 & 70.8/69.8  \\
\hline \hline
\multicolumn{4}{l}{2. Multi-task sentence representation learning} \\ 
\hline
\multicolumn{4}{l}{2.1. 3-datasets and 2-tasks (QQP and SNLI) } \\
% \hline
% 2.1.1. Fully Shared & 86.6 & 84.8 & x \\
2.1.1. Shared Private & 86.8 & 84.7 & x  \\ 
2.1.2. Adversarial Shared Private, $\beta=0.01, \gamma=0.05$ & \underline{\textbf{87.0}} & \underline{84.9} & x    \\ 
\hline
% \hline
\multicolumn{4}{l}{2.2. 3-datasets and 2-tasks (QQP and AllNLI)} \\ 
% \hline
% 2.2.1. Fully Shared & \underline{86.8} & \underline{84.8} & 70.0/68.9 \\
2.2.1. Shared Private & 86.0 & \underline{84.7} & \underline{70.8/69.3}  \\ 
2.2.2. Adversarial Shared Private, $\beta=0.01, \gamma=0.05$ & \underline{86.6} & 84.3 & 69.6/68.3   \\ 
\hline
% \hline
\multicolumn{4}{l}{2.3. 3-datasets and 3-tasks (QQP, SNLI and Multi-NLI)} \\ 
% \hline
% 2.3.1. Fully Shared & 85.9 & 84.3 & 70.1/69.6 \\
2.3.1. Shared Private & \underline{\textbf{87.0}} & \underline{\bf 85.2} & \underline{\bf 71.0/70.1}  \\
2.3.2. Adversarial Shared Private, $\beta=0.005, \gamma=0.001$ & 86.3 & 84.7 & \underline{\bf 71.0/70.1}  \\ 
% \hline 
% \hline
% \multicolumn{4}{l}{3. Multi-task contextualized word vectors learning} \\ 
% % \hline
% 3.1 SNLI + Multi-NLI & x & 85.8 & 73.3/72.3  \\
% 3.2 SNLI + Multi-NLI + QQP & 87.1 & 86.1 & 73.8/72.8  \\
\hline
\end{tabular}
% }
\caption{Test accuracy of the source tasks obtained through various multi-task learning architectures. Underlined values indicate best performance among models trained on the same set of tasks and bold-faced values indicate best performance across the board.
% (excluding block 3).
}
\label{table:source_task_comparison}
% \vspace{-2mm}
\end{table}
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

==> table/table6.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\begin{table*}[h]
\centering
% \resizebox{\linewidth}{!}{%
\small
\begin{tabular}{l c@{} c@{} c@{} c@{} c@{} c}
% \begin{tabular}{l@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{\hskip 0.05in} c@{}}
\hline
Model Type  & \begin{tabular}{c} Length \\ Prediction \end{tabular}  & \begin{tabular}{c} POS tag \\ Prediction \end{tabular} & \begin{tabular}{c} Word \\ Content \end{tabular}  & \begin{tabular}{c} Word \\ Order \end{tabular} & \begin{tabular}{c} WSD \end{tabular} & \begin{tabular}{c@{}} Sentence \\ Ordering \end{tabular}  \\ 
\hline
% Majority vote classifier  & -  & 84.23	& 75.33 & 57.04 \\ 
\hline
\multicolumn{7}{l}{Single-task based sentence representation learning} \\ 
%\hline
InferSent (SNLI) & 72.9 & 96.8 & 79.4 &	65.5 & 39.0 & 79.0/77.3 \\ 
InferSent (All-NLI)   & \textbf{73.8} & 97.0 & \textbf{80.2} & 67.1 & 39.0 & 78.1/76.5 \\
\hline
\hline
\multicolumn{7}{l}{Multi-task based sentence representation learning} \\ 
Shared Private & 66.9 & 96.6 & 79.7 & \textbf{69.7} & 45.6 & 78.6/77.2 \\
Adversarial Shared Private & 69.7 & \textbf{97.1} & 79.1 & 68.3 & \textbf{48.1} & \textbf{79.3/77.7} \\
% \hline
% \hline
% \multicolumn{7}{l}{Contextualized word vectors} \\ 
% %\hline
% CoVe \cite{mccann2017learned}   & \textbf{77.2} & 94.9 & 73.7 & \textbf{70.2} & 46.5 & 75.4/74.9 \\
% ELMo \cite{peters2018elmo}   & 58.1 & \textbf{97.5} & 77.5 & 68.5 & \textbf{66.5} & \textbf{81.1/79.3} \\
\hline

\end{tabular}
% }
\caption{Auxiliary task results for sentence representations learned from the best two single-task and our proposed multi-task models.
% and contextualized word vectors. 
We only consider the shared encoder from the shared private multi-task models for auxiliary task experiments.
% Bold-faced and underlined values denote the best and second best results across the board.
Bold-faced values denote the best results across the board.
}
\label{table:aux_comparison}
% \vspace{-2mm}
\end{table*}
